Using Recurrent Neural Networks to Optimize Dynamical Decoupling for Quantum Memory

We utilize machine learning models which are based on recurrent neural networks to optimize dynamical decoupling (DD) sequences. DD is a relatively simple technique for suppressing the errors in quantum memory for certain noise models. In numerical simulations, we show that with minimum use of prior knowledge and starting from random sequences, the models are able to improve over time and eventually output DD-sequences with performance better than that of the well known DD-families. Furthermore, our algorithm is easy to implement in experiments to find solutions tailored to the specific hardware, as it treats the figure of merit as a black box.

==> dd_sequences.tex <==
\section{Dynamical decoupling sequences}
\label{sec:dd_sequences}
In this section, we are going to list several classes of DD-sequences. We will first explain how to concatenate two sequences, as most long DD-sequences are constructed in this manner.
Given two DD-sequences $A=P_1\cdots P_m$ and $B=Q_1\cdots Q_n$, the concatenated sequence $A[B]$ is
\begin{align*}
A [ B ]=(P_1Q_1)Q_2\cdots Q_n(P_2Q_1)Q_2\cdots Q_n \cdots (P_mQ_1)Q_2\cdots Q_n
\end{align*}
As an example, when we concatenate the length-2 and length-4 sequences $XX$ and $XYXY$, we obtain $IYXYIYXY$.

We will use $P_i$ to represent any Pauli matrix $X$, $Y$ or $Z$, and for $i\neq j$, $P_i \neq P_j$. The families of DD-sequences can then be listed as the following:
\begin{description}
	\item[DD4] are length-4 sequences $P_1 P_2 P_1 P_2$.
	\item[DD8] are length-8 sequences $I P_2 P_1 P_2 I P_2 P_1 P_2$.
	\item[EDD8] are length-8 sequences $P_1 P_2 P_1 P_2 P_2 P_1 P_2 P_1$
	\item[CDD16] are length-16 concatenated sequences $DD4[DD4]$
	\item[CDD32] are length-32 concatenated sequences $DD4[DD8]$ and $DD8[DD4]$
	\item[CDD64] are length-64 concatenated sequences $DD4[CDD16]$ and $DD8[DD8]$
\end{description}
Longer DD-sequences can again be obtained by the concatenation of the ones listed above, and in the ideal situation they provide better and better protection against the noise.
However, with realistic experimental capability, the performance usually saturates at a certain concatenation-level.
Since at this moment we are only optimizing short DD-sequences, the listed ones are sufficient to provide a baseline for our purpose.
One important family we did not include here is the ``Knill DD'' (KDD)~\cite{Ryan2010}, since it requires the use of non-Pauli gates.
It is known that in some experiments, the KDD scheme helps to further increase the performance of CDD-sequences~\cite{Souza2011}.
Thus, an interesting question is when given the freedom of applying non-Pauli gates and choosing variable lengths of the sequences, whether our algorithm could discover a similar strategy.


%, which results in the unitary $U_1= X f_{\tau_d} Y f_{\tau_d} X f_{\tau_d} Y f_{\tau_d}$, where $f_{\tau_d}=e^{-i\tau_d H_0}$ is the time evolution of total noise Hamiltonian $H_0$.
%We can then concatenate $XY_4$ with the length-2 sequence $XX$, simply by setting the total unitary evolution to be $U_2=X U_1 XU_1$.

